Benanza: Automatic $\mu$Benchmark Generation to Compute "Lower-bound" Latency and Inform Optimizations of Deep Learning Models on GPUs

As Deep Learning (DL) models have been increasingly used in latency-sensitive applications, there has been a growing interest in improving their response time. An important venue for such improvement is to profile the execution of these models and characterize their performance to identify possible optimization opportunities. However, the current profiling tools lack the highly desired abilities to characterize ideal performance, identify sources of inefficiency, and quantify the benefits of potential optimizations. Such deficiencies have led to slow characterization/optimization cycles that cannot keep up with the fast pace at which new DL models are introduced. We propose Benanza, a sustainable and extensible benchmarking and analysis design that speeds up the characterization/optimization cycle of DL models on GPUs. Benanza consists of four major components: a model processor that parses models into an internal representation, a configurable benchmark generator that automatically generates micro-benchmarks given a set of models, a database of benchmark results, and an analyzer that computes the "lower-bound" latency of DL models using the benchmark data and informs optimizations of model execution. The "lower-bound" latency metric estimates the ideal model execution on a GPU system and serves as the basis for identifying optimization opportunities in frameworks or system libraries. We used Benanza to evaluate 30 ONNX models in MXNet, ONNX Runtime, and PyTorch on 7 GPUs ranging from Kepler to the latest Turing, and identified optimizations in parallel layer execution, cuDNN convolution algorithm selection, framework inefficiency, layer fusion, and using Tensor Cores.

==> Makefile <==
LATEX=pdflatex
LATEXOPT=--shell-escape
NONSTOP=--interaction=nonstopmode

LATEXMK=latexmk
LATEXMKOPT=-pdf
CONTINUOUS=-pvc

SOURCES=main.tex Makefile $(shell find sections/* -type f)
FIGURES := $(shell find figs/* -type f)

all: force

.refresh:
	touch .refresh

main.pdf: main.tex .refresh $(SOURCES) $(FIGURES)
    $(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
        -pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" main

force:
	touch .refresh
	rm -fr main.pdf
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
		-pdflatex="$(LATEX) $(LATEXOPT) %O %S" main

clean:
	$(LATEXMK) -C main
	rm -f main.pdfsync
	rm -rf *~ *.tmp
	rm -f *.bbl *.blg *.aux *.end *.fls *.log *.out *.fdb_latexmk

once:
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" main

debug:
	$(LATEX) $(LATEXOPT) main

.PHONY: clean force once all

==> plots/layer_type_distribution.tex <==






\begin{figure}
\centering
\begin{scaletikzpicturetowidth}{0.5\textwidth}
\begin{tikzpicture}[scale=\tikzscale]
\begin{axis}[
    ymajorgrids=true,
	x tick label style={
		/pgf/number format/1000 sep=},
    ymajorgrids=true,
    grid style=dashed,
    legend pos=north west,
    legend columns=2,
    ymode=log,
    enlargelimits=0.05,
    log ticks with fixed point,
	ybar interval=0.7,
	ylabel={\tiny Count},
	width=0.4\textwidth,
	height=0.04\textwidth,
	cycle list name=Set1,
	cycle list shift=1,
	ticklabel style = {font=\tiny},
	every axis plot/.append style={fill,draw=none,no markers,font=\tiny},
	xticklabels = { \tiny Conv, \tiny Relu, \tiny BatchNorm, \tiny ElemWise,\tiny Unsqueeze, \tiny Pooling, \tiny Reshape, \tiny Concat, \tiny Gemm, \tiny Dropout, \tiny Flatten, \tiny Transpose, \tiny GlblPool, \tiny LRN, \tiny Softmax, \tiny Scale,DUMMY},
	x tick label style={rotate=45,anchor=east},
    xtick=data,
    bar shift=0pt,
    bar width = 10pt,
    ymin=0,
    legend image code/.code={%
        \draw[#1, draw=none] (0cm,-0.1cm) rectangle (0.2cm,0.1cm);
    },
]
	\addplot[black!20!black,fill=black!80!black] table [x index=0,y index=1,col sep=comma] {dist_layer_types.dat};


\end{axis}
\end{tikzpicture}
\end{scaletikzpicturetowidth}
\caption{The $log$ distribution of layer types across the $30$ models.}
  \label{fig:dist_layer_types}
\end{figure}


==> plots/vgg16.tex <==


\begin{figure*}[ht]
\centering
\begin{scaletikzpicturetowidth}{\textwidth}
\tikzstyle{conv}=[draw,fill=convcolor]
\tikzstyle{max}=[draw,dashed,fill=poolcolor]
\tikzstyle{dropout}=[draw,dashed,fill=dropoutcolor]
\tikzstyle{fc}=[draw,fill=fccolor]
\tikzstyle{input}=[draw,fill=white]
\tikzstyle{output}=[draw,fill=white]
\def \coldist {2.5}
\def \widthb {2}

\newcommand{\vggtext}[1]{\textsf{\fontsize{4}{4} \selectfont  #1}}

\tikzstyle{stateTransition}=[->, thick]

\begin{tikzpicture}[scale=1]
    \draw[->, line width=2pt]
        (1.0+0*\coldist, 0.5) --(1.0+0*\coldist, -2.2) --(2.1+0*\coldist, -2.2) --(2.5+0*\coldist, 0.5)
     -- (1.0+1*\coldist, 0.5) --(1.0+1*\coldist, -2.2) --(2.1+1*\coldist, -2.2) --(2.5+1*\coldist, 0.5)
     -- (1.0+2*\coldist, 0.5) --(1.0+2*\coldist, -2.9) --(2.1+2*\coldist, -2.9) --(2.5+2*\coldist, 0.5)
     -- (1.0+3*\coldist, 0.5) --(1.0+3*\coldist, -2.9) --(2.1+3*\coldist, -2.9) --(2.5+3*\coldist, 0.5)
     -- (1.0+4*\coldist, 0.5) --(1.0+4*\coldist, -2.9) --(2.1+4*\coldist, -2.9) --(2.5+4*\coldist, 0.5)
     -- (1.0+5*\coldist, 0.5) --(1.0+5*\coldist, -4.5);

    \draw[draw=none] (0*\coldist,-0.5) rectangle (1.0,-0.7) node[pos=.5] {\vggtext{$224 \times 224$}};
    \draw[input]     (0*\coldist, 0.0) rectangle (2.0,-0.5) node[pos=.5] {\vggtext{Input}};
    \draw[conv]      (0*\coldist,-0.7) rectangle (2.0,-1.2) node[pos=.5] {\vggtext{CONV $64@3 \times 3 / 1$}};
    \draw[conv]      (0*\coldist,-1.4) rectangle (2.0,-1.9) node[pos=.5] {\vggtext{CONV $64@3 \times 3 / 1$}};

    \draw[draw=none] (1*\coldist,-0.5) rectangle (1*\coldist+\widthb/2,-0.7) node[pos=.5] {\vggtext{$112 \times 112$}};
    \draw[max]       (1*\coldist, 0.0) rectangle (1*\coldist+\widthb,-0.5) node[pos=.5] {\vggtext{POOL $2\times 2 / 1$}};
    \draw[conv]      (1*\coldist,-0.7) rectangle (1*\coldist+\widthb,-1.2) node[pos=.5] {\vggtext{CONV $128@3 \times 3 / 1$}};
    \draw[conv]      (1*\coldist,-1.4) rectangle (1*\coldist+\widthb,-1.9) node[pos=.5] {\vggtext{CONV $128@3 \times 3 / 1$}};

    \draw[draw=none] (2*\coldist,-0.5) rectangle (2*\coldist+\widthb/2,-0.7) node[pos=.5] {\vggtext{$56 \times 56$}};
    \draw[max]       (2*\coldist, 0.0) rectangle (2*\coldist+\widthb,-0.5) node[pos=.5] {\vggtext{POOL $2\times 2 / 1$}};
    \draw[conv]      (2*\coldist,-0.7) rectangle (2*\coldist+\widthb,-1.2) node[pos=.5] {\vggtext{CONV $256@3 \times 3 / 1$}};
    \draw[conv]      (2*\coldist,-1.4) rectangle (2*\coldist+\widthb,-1.9) node[pos=.5] {\vggtext{CONV $256@3 \times 3 / 1$}};
    \draw[conv]      (2*\coldist,-2.1) rectangle (2*\coldist+\widthb,-2.6) node[pos=.5] {\vggtext{CONV $256@3 \times 3 / 1$}};

    \draw[draw=none] (3*\coldist,-0.5) rectangle (3*\coldist+\widthb/2,-0.7) node[pos=.5] {\vggtext{$28 \times 28$}};
    \draw[max]       (3*\coldist,-0.0) rectangle (3*\coldist+\widthb,-0.5) node[pos=.5] {\vggtext{POOL $2\times 2 / 1$}};
    \draw[conv]      (3*\coldist,-0.7) rectangle (3*\coldist+\widthb,-1.2) node[pos=.5] {\vggtext{CONV $512@3 \times 3 / 1$}};
    \draw[conv]      (3*\coldist,-1.4) rectangle (3*\coldist+\widthb,-1.9) node[pos=.5] {\vggtext{CONV $512@3 \times 3 / 1$}};
    \draw[conv]      (3*\coldist,-2.1) rectangle (3*\coldist+\widthb,-2.6) node[pos=.5] {\vggtext{CONV $512@3 \times 3 / 1$}};

    \draw[draw=none] (4*\coldist,-0.5) rectangle (4*\coldist+\widthb/2,-0.7) node[pos=.5] {\vggtext{$14 \times 14$}};
    \draw[max]       (4*\coldist,-0.0) rectangle (4*\coldist+\widthb,-0.5) node[pos=.5] {\vggtext{POOL $2\times 2 / 1$}};
    \draw[conv]      (4*\coldist,-0.7) rectangle (4*\coldist+\widthb,-1.2) node[pos=.5] {\vggtext{CONV $512@3 \times 3 / 1$}};
    \draw[conv]      (4*\coldist,-1.4) rectangle (4*\coldist+\widthb,-1.9) node[pos=.5] {\vggtext{CONV $512@3 \times 3 / 1$}};
    \draw[conv]      (4*\coldist,-2.1) rectangle (4*\coldist+\widthb,-2.6) node[pos=.5] {\vggtext{CONV $512@3 \times 3 / 1$}};

    \draw[draw=none] (5*\coldist,-0.5) rectangle (5*\coldist+\widthb/2,-0.7) node[pos=.5] {\vggtext{$7 \times 7$}};
    \draw[max]       (5*\coldist,-0.0) rectangle (5*\coldist+\widthb,-0.5) node[pos=.5] {\vggtext{POOL $2\times 2 / 1$}};
    \draw[fc]        (5*\coldist,-0.7) rectangle (5*\coldist+\widthb,-1.2) node[pos=.5] {\vggtext{FC $4096$}};
    \draw[dropout]   (5*\coldist,-1.4) rectangle (5*\coldist+\widthb,-1.9) node[pos=.5] {\vggtext{DRP $0.5$}};
    \draw[fc]        (5*\coldist,-2.1) rectangle (5*\coldist+\widthb,-2.6) node[pos=.5] {\vggtext{FC $4096$}};
    \draw[dropout]   (5*\coldist,-2.8) rectangle (5*\coldist+\widthb,-3.3) node[pos=.5] {\vggtext{DRP $0.5$}};
    \draw[output]    (5*\coldist,-3.5) rectangle (5*\coldist+\widthb,-4.0) node[pos=.5] {\vggtext{FC $1000$}};
\end{tikzpicture}

\end{scaletikzpicturetowidth}
\caption{VGG16 Architecture}
  \label{fig:vgg16}
\end{figure*}


==> sections/5.x-use_cases.tex <==


\subsection{Other Use Cases of \dnnscope}\label{sec:use_cases}

The methodology presented affords a few extra use cases:

\subsubsection{System Comparison and Advising}

It is common to ask the question: \textit{given a DL model which system should I use?}
This question might come from a user who wants to purchase the hardware that's ideal for the target model, or a cloud provider who needs to schedule or migrate DL tasks.
An open and continuously evolving performance database (that is possibly crowd sourced) would enable such use case.
Through the database and our ``lower-bound'' metric, we could enable users to find a balance between the latency and cost.
Thus, giving advice as to the most cost-effective system to choose given a model and latency requirements.

\subsubsection{DL Model Performance Similarity Analysis}

There is a plethora of research on characterizing DL workloads, but all take a representative model from each domain class.
Through \dnnscope{} we can generate benchmarks and characterizations for all models within the same domain and classify their utility based on performance.
This clustering allows users to easily weigh the accuracy of models within the same cluster for their target latency requirements.







